Crafty: Efficient, HTM-Compatible Persistent Transactions

Byte-addressable persistent memory, such as Intel/Micron 3D XPoint, is an emerging technology that bridges the gap between volatile memory and persistent storage. Data in persistent memory survives crashes and restarts; however, it is challenging to ensure that this data is consistent after failures. Existing approaches incur significant performance costs to ensure crash consistency. This paper introduces Crafty, a new approach for ensuring consistency and atomicity on persistent memory operations using commodity hardware with existing hardware transactional memory (HTM) capabilities, while incurring low overhead. Crafty employs a novel technique called nondestructive undo logging that leverages commodity HTM to control persist ordering. Our evaluation shows that Crafty outperforms state-of-the-art prior work under low contention, and performs competitively under high contention.

==> design-with-redo-log.tex <==
%auto-ignore
\section{Design with Redo Log}

\mike{Does this design work? Does it have any potential advantages compared with the current (undo-log-based) design?
\mike{Update: Persisting a redo log probably won't work, since it's not in general okay
for the recovery observer to roll forward redo logs,
since persisting the log happens \textbf{before} the transaction has actually executed.}}

\subsection{Algorithm}

Each thread has a log that is an array of <address, oldVal, newVal> tuples. The
log lives in NVRAM (maybe only undo or redo log needs to go in NVRAM?). Each
thread has a (volatile) enum variable called mode that can be either LOGGING or
VALIDATING. Other per-thread variables like logStart (start of current transaction)
and logCurr (current position in transaction) are also volatile.

\mike{The following assumes that the log is infinite and intially zeroed out (\ie, not circular).
Later we deal with a circular log that naturally reuses and overwrites old log entries.}

At start of persistent region:

\begin{small}
\begin{verbatim}  
mode = LOGGING
SETJMP // allow retrying region from beginning
XBEGIN
logCurr = logStart // reset log to beginning
\end{verbatim}
\end{small}

Aborts of the transaction return to the \code{XBEGIN}.
Crafty's abort handler jumps to \code{XBEGIN} unless the transaction has aborted too many times,
in which case it switches to acquiring a single global lock (SGL).
The code for that isn't shown; also not shown: each transaction needs to read and check the SGL.

At each write to persistent memory:

\begin{small}
\begin{verbatim}  
if mode == VALIDATING
  // check log consistency
  if *logCurr != <addr, oldVal, newVal>
    Copy transaction's log entries < logCurr to
      after this transaction's pre-commit entry, and
      continue from there (by updating logCurr & logStart) 
    mode = LOGGING
if mode == LOGGING
  *logCurr = <addr, *addr, newVal>
logCurr++
*addr = newVal // the original program write
\end{verbatim}
\end{small}

\textcolor{blue}{Alternate design: Avoid the conditional logic at each write, and instead do all the validation at the end of the transaction.}

At end of persistent region:

\begin{small}
\begin{verbatim}  
if mode == VALIDATING
  if *logCurr is a PRECOMMIT entry
    // we can commit, yay
    *logCurr = <COMMIT, _, RDTSC()> // overwrite pre-commit entry
    XEND
    CWLB of *logCurr
    CLWB of each *addr s.t. <addr, oldVal, newVal> in
                            *logStart to *(logCurr-1)
    logCurr++
  else
    Copy transaction's log entries < logCurr to
      after this transaction's pre-commit entry, and
      continue from there (by updating logCurr & logStart) 
    mode = LOGGING
if mode == LOGGING
  // roll back writes:
  foreach <addr, oldValue, newValue>
          from *(logCurr-1) to *logStart in rev. order
    *addr = oldValue // revert to old value
  *(logCurr++) = <PRECOMMIT, RDTSC(), 0>
  XEND
  CLWB of each cache line in range [*logStart, *logCurr)
  // omit SFENCE here: next txn provides fence behavior
  mode = VALIDATING
  LONGJMP // retry region
\end{verbatim}
\end{small}

\mike{Kaan points out that for the last transaction $\mathit{txn}$ committed in a thread $T$---which
we can't be sure has actually persisted (\eg, the CLWBs following the "VALIDATION" transaction
will not necessarily execute within bounded time, and there's not necessarily a knowable time bound on
how long it takes for the CLWBs to finish persisting---it's incorrect for another thread $T'$ to overwrite
an entry for its old transaction $\mathit{txn}'$ in $T'$ log if $\ts_{\mathit{txn}'} > \ts_{\mathit{txn}}$.
Previously it seemed that recovery could roll forward $\mathit{txn}$, but that might conflict with writes performed
(later) by $\mathit{txn}'$, which recovery won't be able to also roll forward since $T'$ has overwritten $\mathit{txn}'$ in the log.
\medskip\\
We discussed how $T'$ could periodically (every time it reuses half the log?)
make sure that no transaction like $\mathit{txn}$ exists.
If a transaction like $\mathit{txn}$ exists, $T'$ can go ahead and persist $\mathit{txn}$ itself.
We thought it would be complicated to have another thread writing to a thread's mostly-private log,
but on further thought I think we can use transactions to do it safely and relatively simply.
\medskip\\
Is there now any point in having a redo log (\ie, having redo entries in the log)?
It seems like redo entries are not only unnecessary in the persistent log,
but they may not be needed at all.}

\mike{Update: The ``we don't know when committed writes from the latest transaction will actually persist'' issue actually creates two problems:
\begin{enumerate}
\item Reusing log entries (\eg, in a circular log) means that another thread may overwrite entries that make consistent recovery impossible.
\item Recovery might need to roll back an arbitrarily old transaction.
\end{enumerate}
Using an ``undo log only'' solution won't fix the second problem,
but a ``redo log only'' solution would. I don't think there's any need for both undo and redo entries,
so at this point I'm thinking a redo log makes sense.
Of course, to support rolling back a transaction in LOGGING mode, a transaction needs at least a temporary undo log.
To minimize transaction and cache footprint,
a transaction in LOGGING mode would actually write undo entries into the redo log,
and rollback before transaction commit would overwrite the entries with redo entries while rolling back.
\medskip\\
Then we still need a way to handle reuse of log entries / circular logs.
I think it'll work to have a thread $T$ periodically (twice per log length) check
that it's not running too far ahead of any other thread
(in particular, that $T$ is not in danger of overwriting a log entry that comes after thread $U$'s latest transaction,
whose writes haven't necessarily persisted),
using an optimization that usually allows reading just one global timestamp.
If $T$ is in danger of overwriting such a log entry, it first goes ahead and persists $U$'s latest transaction's writes.}

\mike{Update \#2: On second thought, can a redo log really work in this case?
In particular, it doesn't possible to persist the ``transaction redo log is complete'' status
atomically with the successful termination of the VALIDATION transaction.
For example, if recovery sees a fully persisted committed transaction of redo entries,
it doesn't know whether the VALIDATION transaction didn't commit (implying roll forward would be wrong)
or if some program writes persisted (in which case roll forward is necessary).
\medskip\\
Assuming that's right, then the log needs to have undo entries.
And we should try to solve both problems above with one solution
that avoids both the recovery point being too far in the past and
reusing log entries that are needed for recovery.}

\subsection{Recovery}

The following refers to \emph{fully persisted} pre-committed or committed transactions,
which means that all of the entries in the transaction have fully persisted,
including, the pre-commit or commit entry.
So far we have assumed an infinite log that is initially zeroed
(no wraparound or reuse) and that each entry is entirely on a single cache line.
In this case, detecting fully persisted entries and thus transactions is straightforward:
they are identifiable by virtue of being nonzero.

Later we define how to detect fully persisted entries (and thus transactions)
in the context of a circular log and entries that can span cache lines.

\paragraph{Recovery algorithm.}

\begin{enumerate}

\item
For each thread:
Find the latest pre-committed or committed transaction,
by finding the PRECOMMIT or COMMIT entry with the latest timestamp.
If the algorithm finds a PRECOMMIT entry, check that every entry in the transaction has persisted,
by checking the wraparound bit; and,
if the PRECOMMIT entry's addr (wraparound bit) and oldValue (timestamp) fields are on different cache lines,
check the following entry's wraparound bit to ensure the PRECOMMIT entry has fully persisted).
If the algorithm finds a COMMIT entry, it has fully persisted as long as the newValue (commit timestamp) field
is nonzero.

\item
For each thread $T$:
Let $\mathit{maxTS}_T$ be the timestamp of $T$'s latest fully persisted pre-committed or committed transaction.
\mike{If $T$'s latest fully persisted transaction is only pre-committed,
should $\mathit{maxTS}_T$ instead be set to $(\textnormal{timestamp} - 1)$?}

\item
Let $\mathit{recoveryTS} = \min_{\forall T}(\mathit{maxTS}_T)$ be the \emph{recovery timestamp}.

\item
For all transactions $\mathit{txn}$ that such that $\mathit{ts}_\mathit{txn} > \mathit{recoveryTS}$
(which should include any transaction that is only fully persisted as a pre-committed transaction),
roll back the transactions, in reverse timestamp order,
\mike{If rolling back a transaction fully persisted as a committed transaction,
use the pre-commit or commit timestamp?}
by setting \code{*addr = oldValue} for the transaction's log entries in reverse order.

\item
For all transactions $\mathit{txn}$ fully persisted as committed transactions,
such that $\mathit{ts}_\mathit{txn} \le \mathit{recoveryTS}$,
roll \emph{forward} the transactions, in forward timestamp order,
by setting \code{*addr = newValue} for the transaction's log entries in forward order.
Because this step is only needed in case a committed transaction's writes have not fully persisted,
we only need to roll forward a transaction if it is a thread's
\emph{last} fully persisted transaction (no fully persisted pre-committed or committed
transaction follows the transaction in the log).
\mike{Hmm, we don't want to end up overwriting newer values with older values.
We should probably roll forward any transaction that has a greater timestamp
(subject to $\mathit{ts}_\mathit{txn} \le \mathit{recoveryTS}$)
than any rolled-forward transaction.}

\end{enumerate}
% %
Assuming CLWB (without SFENCE) persists within bounded time, only a bounded
number of transactions must be rolled back for any thread, allowing for bounded
(circular) logs.

\subsection{Handling High-Performance Logs}

As presented so far, the algorithm assumes that log entries are initially cleared (zeroed)
and that a log entry <addr, oldValue, newValue> will fit entirely on one cache line.
However, for performance reasons, we would like to violate both of these assumptions:
(1) to improve cache locality and make it easier to reuse the memory for old log entries,
an implementation will likely use a circular log, and
(2) to save space, an implementation may pack
log entries, causing some entries to span two cache lines
(\eg, if addr, oldValue, and newValue are each 8 bytes, then each log entry is 24 bytes,
so some entries will span 2$^k$-byte cache lines).

To handle a circular log and differentiate cache lines written after versus before the latest log wraparound,
we use a per-thread \emph{wraparound} bit that flips each time the log wraps around~\cite{logging-algorithms-oopsla17}.
Each written log entry includes the value of the wraparound bit.
Assuming CLWB+SFENCE occurs at least as often as wraparound,
recovery can only observe log entries that are after the next-to-latest wraparound,
so a single wraparound bit suffices.

To store the wraparound bit,
we can ``steal'' the low bits of the \code{addr} element of each log entry.
A PRECOMMIT/COMMIT entry uses 
an \code{addr} value that also leaves bits available for storing the wraparound bit's current value.
As long as entries (24 bytes in our implementation) are smaller than cache lines (\eg, 64 bytes in our experiments),
every cache line will have at least one wraparound bit.

Despite this property, a remaining challenge is that the wraparound bit is at the beginning
of an entry; what if some or all of the rest of the entry is on another cache line?
This is only a problem for PRECOMMIT/COMMIT entries, since other entries have some other
entry following them from the same transaction, which can be used to check for persistence of the cache line.
If a PRECOMMIT/COMMIT entry spans a cache line
(so the \code{newValue} field and possibly the \code{oldValue} field
are on a different cache line than the \code{addr} field),
then recovery will not be able to differentiate between fields from old (before wraparound)
and new entries.
We solve this problem by setting the \code{newValue} field of the PRECOMMIT entry
to either 0 or 1---whatever the flip of the lowest bit of the prior value in that word is.
We expand PRECOMMIT into two tags: PRECOMMIT\_PARITY\_EVEN indicating that the updated
\code{newValue} is 0, and PRECOMMIT\_PARITY\_ODD indicating that the updated \code{newValue} is 1.
Recovery can determine if a pre-commit entry is fully persisted by checking if the
pre-commit tag (PRECOMMIT\_PARITY\_EVEN or PRECOMMIT\_PARITY\_ODD) matches \code{newValue}.
% The implementation solves this issue by setting the \code{addr} field of
% the \emph{following} log entry's \code{addr} field to a special DUMMY value (ORed with the wraparound bit).
% If recovery observes a PRECOMMIT entry that spans a cache line,
% it can check the next entry's \code{addr}'s wraparound bit to determine if the
% undo log for a transaction has completely persisted (in addition, all other entries' wraparound bits
% must have the correct value).
Recovery can tell the difference between a partially and fully
persisted \COMMITTED entry by checking the \code{newValue} entry, which will either have 0 or 1
(indicating pre-commit) or a value $\ge$ 2 (indicating a timestamp; we assume timestamps start at 2).


==> old-algorithm.tex <==
%auto-ignore
\section{Old Low-Level Description of \Crafty's Execution of Persistent Regions}

Each thread has a log that is an array of <address, oldVal> pairs. The
log lives in NVRAM. Each
thread has a (volatile) enum variable called mode that can be either LOGGING or
VALIDATING. Other per-thread variables like logStart (start of current transaction)
and logCurr (current position in transaction) are also volatile.

The following assumes that the log is intially zeroed out and not reused (\ie, not circular).
Later we deal with a circular log that naturally reuses and overwrites old log entries.

At start of persistent region:

\begin{small}
\begin{verbatim}  
mode = LOGGING
SETJMP // allow retrying region from beginning
XBEGIN
logCurr = logStart // reset log to beginning
\end{verbatim}
\end{small}

Aborts of the transaction return to the \code{XBEGIN}.
Crafty's abort handler jumps to \code{XBEGIN} unless the transaction has aborted too many times,
in which case it switches to acquiring a single global lock (SGL).
The code for that isn't shown; also not shown: each transaction needs to read and check the SGL.

At each write to persistent memory:

\begin{small}
\begin{verbatim}  
if mode == VALIDATING
  // check log consistency
  if *logCurr != <addr, oldVal>
    Copy transaction's log entries < logCurr to
      after this transaction's commit entry, and
      continue from there (by updating logCurr & logStart) 
    mode = LOGGING
if mode == LOGGING
  *logCurr = <addr, *addr>
logCurr++
*addr = newVal // the original program write
\end{verbatim}
\end{small}

At end of persistent region:

% \mike{I think the algorithm may need to update the timestamp for a successfully validated transaction,
% In particular, if recovery decides it can keep a transaction based on it not being a thread's last
% transaction and the timestamp being late enough,
% then it could incorrectly think a committed transaction is older than it really is,
% leading to an inconsistent state w.r.t.\ the other transactions.
% In the following example, in which T1's logging and validating of a transaction are interleaved by
% another transaction's logging and validation. In the example (all values initially 0), what if recovery
% thinks it must roll back T2's transaction but that it doesn't need to also roll back T1's <COMMIT,1>
% because it's so old.
% However, that'd give x=1, z=1, y=0 as the recovery state, which seems incorrect.}
% \kaan{I agree. Another solution would be to reintroduce the redo log (which can be in
%   volatile memory). That way, the validation would fail and T1 would restart its
%   log. Updating the timestamp is simpler, so I'll go with that.}

% \begin{verbatim}
% T1            T2
% --            --
% LOGGING:
% x=1 <&x, 0>
% z=y <&z, 0>
% <COMMIT,1>
%                LOGGING:
%                y = 1 <&y, 0>
%                <COMMIT,2>
%                VALIDATING:
%                y = 1
%                Successfully validates

% VALIDATING:
% x=1
% z=y
% Successfully validates
% ...
% <COMMIT,4> // from another transaction
% \end{verbatim}

\begin{small}
\begin{verbatim}
if mode == VALIDATING
  if *logCurr is a COMMIT entry
    // Log is valid, finish persistent region
    *logCurr = <_, RDTSC()> // update COMMIT timestamp
    logStart = logCurr + 1 // ready for next transaction
    XEND
    CLWB of *logCurr
    CLWB of each *addr s.t. <addr, oldVal> in
                            *logStart to *(logCurr-1)
  else // if LOGGING transaction executed more writes
    Copy transaction's log entries < logCurr to
      after this transaction's commit entry, and
      continue from there (by updating logCurr & logStart)
    mode = LOGGING
if mode == LOGGING
  if logCurr != logStart // non-read-only transaction?
    // roll back writes:
    foreach <addr, oldValue>
            from *(logCurr-1) to *logStart in rev. order
      *addr = oldValue // revert to old value
    *(logCurr++) = <COMMIT, RDTSC()>
    XEND
    CLWB of each cache line in [*logStart, *logCurr)
    // omit SFENCE here: next txn provides fence behavior
    mode = VALIDATING
    LONGJMP // retry region
\end{verbatim}
\end{small}

\paragraph{Optimistically committing writes.}

After a LOGGING mode transaction, a transaction can commit its writes,
as long as no other transaction makes progress in the meantime:

\noindent
\begin{minipage}{\linewidth}
\begin{small}
\begin{verbatim}
if mode == VALIDATING
  ...
if mode == LOGGING
  if logCurr != logStart // non-read-only transaction?
    // roll back writes:
    foreach <addr, oldValue>
            from *(logCurr-1) to *logStart in rev. order
      *addr = oldValue // revert to old value
      // also construct a volatile redo log here
      currThreadLastLog = RDTSC()
      *(logCurr++) = <COMMIT, currThreadLastLog>
    XEND
    CLWB of each cache line in [*logStart, *logCurr)
    // omit SFENCE here: next txn provides fence behavior
    if (gLastCopy < currThreadLastLog) { // possible optimization
      XBEGIN
      if (gLastCopy < currThreadLastLog) {
        Perform writes using redo log
        gLastCopy = RDTSC()
      } else {
        XABORT
      }
      XEND
    }
    if (didn't commit a copy transaction) {
      mode = VALIDATING
      LONGJMP // retry region
    }
\end{verbatim}
\end{small}
\end{minipage}

\notes{
\paragraph{Alterate design.}

Instead, we could avoid the conditional logic at each write, and do all validation at the end of the transaction.
That'd probably require creating a second copy of the logged transaction, although it perhaps could be in volatile memory.
}

\paragraph{Optimizations.}

When a transaction in LOGGING mode commits, if it has performed no writes to persistent memory,
then it does not need to log writes or a COMMIT entry, and does not need to repeat the transaction in VALIDATION mode.
The pseudocode above handles the read-only case by checking \code{logCurr != logStart}.

\paragraph{Single global lock (SGL) fallback.}

A transaction may repeatedly fail to commit because of conflicts with other transactions
or because the transaction is so long it can't make progress or contains events that aren't allowed in transactions.
Assuming HTM is also the concurrency control mechanism, it will fall back to the SGL.

If Crafty executes an SGL-guarded atomic region non-transactionally,
then it needs to persist each undo log write individually (right?),
which will perform poorly compared with related solutions such as NV-HTM,
which still amortize persist latency even for SGL-guarded regions.

Alternatively, Crafty should try to execute an SGL-guarded region transactionally.
If that fails, Crafty should try to execute a subset of the region (based on counting writes)
transactionally, decreasing the subset size when aborts happen.

Related but more general:
Does a transaction with a single write actually need to use a transaction to provide persistence?
\kaan{No, assuming the program is race-free, it just needs two flushes: one before writing the log and one after. The one before the log ensures that the writes of the previous transaction have persisted (recovery assumes they have persisted), and the other one orders the log to the write in current one-write "transaction".}
Can a Crafty transaction wait until the first write to actually start the HTM transaction
(might be needed to get transactions to succeed inside of SGL-guarded regions)?
\kaan{Crafty can wait until the first write or read to persistent memory.}



==> results-SGL-retry-bit-comparison.tex <==
%auto-ignore
\begin{table}
\small
\begin{tabular}{@{}l|rrrrr@{}}
Solution & 1 & 2 & 4 & 8 & 12 \\
\hline
 & \mc{4}{c}{genome} \\
HTM-only & 22.08  & 16.81  & 14.75  & 12.34  & 11.98 \\
DudeTM & 25.88  & 20.26  & 16.35  & 12.72  & 12.75 \\
NV-HTM & 27.26  & 22.68  & 17.11  & 13.73  & 12.79 \\
Crafty & 22.60  & 17.48  & 14.98  & 12.29  & 12.29 \\
\hline
 & \mc{4}{c}{intruder} \\
HTM-only & 37.95  & 22.80  & 14.10  & 12.26  & 13.46 \\
DudeTM & 86.36  & 50.87  & 29.32  & 20.36  & 21.24 \\
NV-HTM & 87.40  & 51.81  & 28.95  & 18.86  & 19.73 \\
Crafty & 60.09  & -  & -  & 18.36  & 22.42 \\
\hline
 & \mc{4}{c}{kmeans-high} \\
HTM-only & 0.53  & 0.42  & 0.35  & 0.27  & 0.24 \\
DudeTM & 2.85  & 1.50  & 0.80  & 0.57  & 0.53 \\
NV-HTM & 2.78  & 1.54  & 0.86  & 0.62  & 0.55 \\
Crafty & 1.84  & 1.12  & 0.58  & 0.47  & 0.47 \\
\hline
 & \mc{4}{c}{kmeans-low} \\
HTM-only & 1.19  & 0.67  & 0.42  & 0.34  & 0.32 \\
DudeTM & 3.52  & 1.87  & 0.98  & 0.66  & 0.62 \\
NV-HTM & 3.45  & 1.89  & 1.01  & 0.74  & 0.64 \\
Crafty & 2.71  & 1.32  & 0.72  & 0.51  & 0.50 \\
\hline
 & \mc{4}{c}{ssca2} \\
HTM-only & 23.00  & 11.35  & 5.48  & 2.86  & 2.32 \\
DudeTM & 84.34  & 47.85  & 24.92  & 20.19  & 17.26 \\
NV-HTM & 84.43  & 45.96  & 24.64  & 16.54  & 11.79 \\
Crafty & 41.89  & 22.19  & 10.97  & 5.52  & 3.90 \\
\hline
 & \mc{4}{c}{vacation-high} \\
HTM-only & 56.98  & 34.75  & 22.03  & 24.16  & 32.43 \\
DudeTM & 77.35  & 47.14  & 28.85  & 24.57  & 30.48 \\
NV-HTM & 73.00  & 46.79  & 28.50  & 24.12  & 29.06 \\
Crafty & 71.84  & 52.69  & 33.91  & 30.21  & 34.99 \\
\hline
 & \mc{4}{c}{vacation-low} \\
HTM-only & 41.80  & 23.14  & 12.85  & 13.21  & 20.73 \\
DudeTM & 58.87  & 33.43  & 17.79  & 14.26  & 18.34 \\
NV-HTM & 57.96  & 32.85  & 17.48  & 13.09  & 17.47 \\
Crafty & 59.08  & 38.11  & 21.01  & 18.46  & 22.87 \\
\hline
 & \mc{4}{c}{yada} \\
HTM-only & 17.99  & 21.88  & 19.05  & 17.37  & 18.22 \\
DudeTM & 33.40  & 26.47  & 20.47  & 18.16  & 19.14 \\
NV-HTM & 32.93  & 26.16  & 20.50  & 18.06  & 19.01 \\
Crafty & 21.34  & -  & -  & -  & - \\

\end{tabular}
\caption{Execution times when the capacity bit being set switches to SGL.
\label{tab:time-retry-SGL}}
\end{table}

\begin{table}
\small
\begin{tabular}{@{}l|rrrrr@{}}
Solution & 1 & 2 & 4 & 8 & 12 \\
\hline
 & \mc{4}{c}{genome} \\
HTM-only & 12.30  & 14.83  & 12.84  & 11.57  & 12.99 \\
DudeTM & 16.22  & 13.95  & 14.00  & 12.70  & 13.18 \\
NV-HTM & 16.53  & 14.83  & 13.82  & 13.14  & 14.14 \\
Crafty & 12.08  & 14.99  & 13.16  & 12.48  & 13.96 \\
\hline
 & \mc{4}{c}{intruder} \\
HTM-only & 37.16  & 26.17  & 21.90  & 20.49  & 43.27 \\
DudeTM & 84.28  & 51.96  & 32.61  & 23.70  & 33.85 \\
NV-HTM & 85.90  & 54.05  & 34.30  & 23.38  & 31.27 \\
Crafty & 52.72  & 36.17  & 28.70  & 33.29  & 46.10 \\
\hline
 & \mc{4}{c}{kmeans-high} \\
HTM-only & 0.53  & 0.32  & 0.34  & 0.26  & 0.22 \\
DudeTM & 2.78  & 1.47  & 0.77  & 0.55  & 0.51 \\
NV-HTM & 2.75  & 1.48  & 0.78  & 0.58  & 0.53 \\
Crafty & 0.98  & 0.76  & 0.53  & 0.41  & 0.37 \\
\hline
 & \mc{4}{c}{kmeans-low} \\
HTM-only & 1.18  & 0.64  & 0.38  & 0.34  & 0.35 \\
DudeTM & 3.48  & 1.84  & 0.95  & 0.63  & 0.59 \\
NV-HTM & 3.42  & 1.84  & 0.96  & 0.68  & 0.62 \\
Crafty & 1.64  & 0.93  & 0.68  & 0.53  & 0.57 \\
\hline
 & \mc{4}{c}{ssca2} \\
HTM-only & 23.39  & 12.18  & 6.57  & 5.12  & 9.27 \\
DudeTM & 85.05  & 46.55  & 24.68  & 17.51  & 12.63 \\
NV-HTM & 85.49  & 47.62  & 25.04  & 17.08  & 12.17 \\
Crafty & 40.97  & 22.25  & 11.89  & 7.49  & 13.73 \\
\hline
 & \mc{4}{c}{vacation-high} \\
HTM-only & 54.01  & 38.19  & 31.47  & 32.16  & 48.38 \\
DudeTM & 71.74  & 47.57  & 35.41  & 32.61  & 48.39 \\
NV-HTM & 70.75  & 48.30  & 35.84  & 31.17  & 46.92 \\
Crafty & 58.17  & 43.14  & 37.08  & 37.67  & - \\
\hline
 & \mc{4}{c}{vacation-low} \\
HTM-only & 40.07  & 25.81  & 19.77  & 20.27  & 35.65 \\
DudeTM & 54.30  & 34.25  & 24.35  & 21.07  & 36.20 \\
NV-HTM & 54.13  & 33.94  & 23.93  & 19.96  & 33.59 \\
Crafty & 44.59  & 31.10  & 24.57  & 25.57  & - \\
\hline
 & \mc{4}{c}{yada} \\
HTM-only & 17.49  & 19.11  & 18.56  & 17.91  & 19.12 \\
DudeTM & 32.45  & 24.22  & 19.79  & 18.76  & 19.92 \\
NV-HTM & 31.77  & 23.78  & 19.65  & 18.45  & 19.57 \\
Crafty & 19.94  & -  & -  & -  & - \\
\end{tabular}
\caption{Execution times when the retry bit being clear switches to SGL.}
\end{table}



\begin{table}
    \small
    \begin{tabular}{@{}l|rrrrr@{}}
    Solution & 1 & 2 & 4 & 8 & 12 \\
    
    \hline
    & \mc{4}{c}{genome} \\
   HTM-only & 13.65  & 15.35  & 13.12  & 12.02  & 12.84 \\
   DudeTM & 17.16  & 14.87  & 14.09  & 12.74  & 12.79 \\
   NV-HTM & 17.92  & 15.18  & 14.04  & 13.10  & 13.49 \\
   Crafty & 13.74  & 15.84  & 13.68  & 12.82  & 13.27 \\
   \hline
    & \mc{4}{c}{intruder} \\
   HTM-only & 39.47  & 27.12  & 18.77  & 11.55  & 10.02 \\
   DudeTM & 86.85  & 53.81  & 34.38  & 21.54  & 20.27 \\
   NV-HTM & 88.52  & 54.58  & 33.97  & 19.78  & 17.99 \\
   Crafty & 55.73  & 40.53  & 32.29  & 21.88  & 22.91 \\
   \hline
    & \mc{4}{c}{kmeans-high} \\
   HTM-only & 0.58  & 0.37  & 0.39  & 0.33  & 0.32 \\
   DudeTM & 2.79  & 1.50  & 0.78  & 0.57  & 0.53 \\
   NV-HTM & 2.78  & 1.50  & 0.81  & 0.61  & 0.56 \\
   Crafty & 0.95  & 0.70  & 0.54  & 0.47  & 0.48 \\
   \hline
    & \mc{4}{c}{kmeans-low} \\
   HTM-only & 1.24  & 0.68  & 0.41  & 0.37  & 0.39 \\
   DudeTM & 3.50  & 1.86  & 0.99  & 0.66  & 0.62 \\
   NV-HTM & 3.46  & 1.88  & 1.00  & 0.71  & 0.64 \\
   Crafty & 1.60  & 0.90  & 0.63  & 0.51  & 0.53 \\
   \hline
    & \mc{4}{c}{ssca2} \\
   HTM-only & 23.60  & 12.21  & 6.18  & 3.66  & 2.99 \\
   DudeTM & 83.99  & 47.31  & 25.26  & 20.41  & 16.92 \\
   NV-HTM & 83.79  & 47.88  & 25.04  & 16.95  & 11.86 \\
   Crafty & 40.63  & 22.06  & 12.25  & 6.86  & 5.85 \\
   \hline
    & \mc{4}{c}{vacation-high} \\
   HTM-only & 67.46  & 40.22  & 31.29  & 25.46  & 26.03 \\
   DudeTM & 83.14  & 49.88  & 35.35  & 28.17  & 27.34 \\
   NV-HTM & 88.15  & 52.26  & 37.48  & 30.17  & 28.37 \\
   Crafty & 79.04  & 47.72  & 35.55  & 30.86  & 31.01 \\
   \hline
    & \mc{4}{c}{vacation-low} \\
   HTM-only & 42.99  & 25.88  & 18.96  & 15.06  & 14.75 \\
   DudeTM & 55.24  & 33.89  & 23.06  & 17.22  & 15.97 \\
   NV-HTM & 57.03  & 35.44  & 25.48  & 18.50  & 17.51 \\
   Crafty & 51.25  & 32.18  & 24.30  & 20.56  & 19.80 \\
   \hline
    & \mc{4}{c}{yada} \\
   HTM-only & 46.98  & 21.53  & 18.49  & 17.89  & 18.89 \\
   DudeTM & 60.42  & 26.63  & 19.95  & 18.69  & 19.85 \\
   NV-HTM & 61.55  & 26.73  & 20.19  & 18.84  & 19.73 \\
   Crafty & 46.60  & -  & -  & -  & - \\
    
    \end{tabular}
    \caption{Execution times when the status code being 0 switches to SGL.}
    \end{table}
    

    \begin{table}
        \small
        \begin{tabular}{@{}l|rrrrr@{}}
        Solution & 1 & 2 & 4 & 8 & 12 \\
        
        \hline
        & \mc{4}{c}{genome} \\
       HTM-only & 22.00  & 17.02  & 14.80  & 11.75  & 11.74 \\
       DudeTM & 25.32  & 20.10  & 15.63  & 12.34  & 12.07 \\
       NV-HTM & 26.80  & 22.36  & 16.88  & 13.11  & 12.47 \\
       Crafty & 23.13  & 17.68  & 14.86  & 11.96  & 11.66 \\
       \hline
        & \mc{4}{c}{intruder} \\
       HTM-only & 43.08  & 26.12  & 14.24  & 8.58  & 6.65 \\
       DudeTM & 91.31  & 51.99  & 28.60  & 17.27  & 15.04 \\
       NV-HTM & 92.99  & 52.94  & 28.89  & 15.78  & 13.11 \\
       Crafty & 68.28  & 41.71  & 25.81  & 16.09  & 16.55 \\
       \hline
        & \mc{4}{c}{kmeans-high} \\
       HTM-only & 0.62  & 0.53  & 0.39  & 0.33  & 0.33 \\
       DudeTM & 2.82  & 1.53  & 0.80  & 0.58  & 0.54 \\
       NV-HTM & 2.84  & 1.63  & 0.84  & 0.62  & 0.56 \\
       Crafty & 1.88  & 1.18  & 0.61  & 0.49  & 0.47 \\
       \hline
        & \mc{4}{c}{kmeans-low} \\
       HTM-only & 1.24  & 0.76  & 0.48  & 0.36  & 0.43 \\
       DudeTM & 3.53  & 1.88  & 0.98  & 0.67  & 0.63 \\
       NV-HTM & 3.49  & 1.91  & 1.00  & 0.70  & 0.64 \\
       Crafty & 2.62  & 1.50  & 0.78  & 0.57  & 0.56 \\
       \hline
        & \mc{4}{c}{ssca2} \\
       HTM-only & 22.33  & 11.34  & 5.54  & 2.99  & 2.30 \\
       DudeTM & 85.48  & 47.13  & 24.53  & 20.36  & 17.03 \\
       NV-HTM & 85.41  & 46.84  & 24.57  & 16.55  & 11.73 \\
       Crafty & 42.11  & 21.68  & 10.68  & 5.56  & 3.96 \\
       \hline
        & \mc{4}{c}{vacation-high} \\
       HTM-only & 79.70  & 39.12  & 19.05  & 18.07  & 19.53 \\
       DudeTM & 96.54  & 52.86  & 28.20  & 22.73  & 20.03 \\
       NV-HTM & 106.94  & 57.01  & 29.23  & 24.03  & 21.36 \\
       Crafty & 145.60  & 77.01  & 40.37  & 26.86  & 24.96 \\
       \hline
        & \mc{4}{c}{vacation-low} \\
       HTM-only & 44.19  & 22.75  & 10.82  & 7.77  & 9.18 \\
       DudeTM & 59.68  & 33.06  & 17.08  & 11.77  & 9.96 \\
       NV-HTM & 62.98  & 32.68  & 16.93  & 12.16  & 10.35 \\
       Crafty & 80.14  & 42.09  & 21.96  & 15.55  & 14.04 \\
       \hline
        & \mc{4}{c}{yada} \\
       HTM-only & 77.44  & 32.06  & 18.64  & 16.80  & 18.01 \\
       DudeTM & 83.41  & 38.88  & 20.82  & 17.77  & 18.86 \\
       NV-HTM & 84.26  & 40.08  & 21.66  & 18.17  & 18.65 \\
       Crafty & 70.41  & -  & -  & -  & - \\
        
        \end{tabular}
        \caption{Execution times of the original configuration.}
        \end{table}


==> results-atom.tex <==
%auto-ignore

    \begin{table*}
    \small
    \begin{tabular}{@{}l|rrrrr@{}}
    Solution & 1 & 2 & 4 & 8 & 12 \\
    
\hline
 & \mc{4}{c}{bayes} \\
HTM-only & 57.25  & 60.12  & 222.84  & 83.11  & 65.72 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 57.55  & 45.12  & 77.90  & 58.24  & 57.10 \\
Crafty & 59.49  & 67.25  & 62.61  & 85.75  & 108.79 \\
\hline
 & \mc{4}{c}{genome} \\
HTM-only & 13.59  & 8.45  & 4.56  & 2.29  & 2.13 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 14.00  & 11.46  & 5.37  & 2.71  & 1.97 \\
Crafty & 21.21  & 8.62  & 4.08  & 2.83  & 2.81 \\
\hline
 & \mc{4}{c}{intruder} \\
HTM-only & 24.51  & 13.82  & 7.83  & 4.73  & 3.96 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 59.16  & 33.38  & 18.50  & 10.24  & 7.47 \\
Crafty & 35.79  & -  & -  & -  & - \\
\hline
 & \mc{4}{c}{kmeans-high} \\
HTM-only & 0.48  & 0.30  & 0.34  & 0.26  & 0.26 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 2.24  & 1.29  & 0.76  & 0.50  & 0.38 \\
Crafty & 0.85  & 0.52  & 1.21  & 1.30  & 1.43 \\
\hline
 & \mc{4}{c}{kmeans-low} \\
HTM-only & 1.14  & 0.65  & 0.39  & 0.30  & 0.26 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 2.88  & 1.66  & 0.95  & 0.56  & 0.42 \\
Crafty & 1.51  & 0.84  & 1.22  & 1.21  & 1.28 \\
\hline
 & \mc{4}{c}{labyrinth} \\
HTM-only & 100.63  & 106.71  & 114.00  & 117.16  & 117.44 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 100.70  & 106.68  & 113.84  & 117.39  & 117.61 \\
Crafty & 103.68  & 105.37  & 113.50  & 117.55  & 117.98 \\
\hline
 & \mc{4}{c}{ssca2} \\
HTM-only & 10.25  & 5.42  & 2.94  & 1.61  & 1.18 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 55.93  & 31.08  & 17.24  & 9.40  & 6.63 \\
Crafty & 51.71  & 29.27  & 15.24  & 7.91  & 3.96 \\
\hline
 & \mc{4}{c}{vacation-high} \\
HTM-only & 41.73  & 22.34  & 12.95  & 8.00  & 9.42 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 55.58  & 31.47  & 18.51  & 10.08  & 7.55 \\
Crafty & 51.38  & 28.59  & 17.20  & 13.00  & 18.56 \\
\hline
 & \mc{4}{c}{vacation-low} \\
HTM-only & 23.46  & 12.40  & 6.92  & 4.03  & 3.64 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 33.32  & 18.34  & 10.36  & 5.79  & 4.08 \\
Crafty & 28.42  & 15.92  & 9.86  & 7.55  & 10.84 \\
\hline
 & \mc{4}{c}{yada} \\
HTM-only & 74.38  & 28.52  & 16.11  & 15.45  & 15.54 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 83.94  & 35.87  & 20.22  & 16.22  & 16.00 \\
Crafty & 69.94  & 39.28  & 29.87  & 36.13  & 42.92 \\

    \end{tabular}
    \caption{Execution times on atom.}
    \end{table*}
    

    \begin{table*}
    \small
    \begin{tabular}{@{}l|rrrrr@{}}
    Solution & 1 & 2 & 4 & 8 & 12 \\
    
\hline
 & \mc{4}{c}{bayes} \\
HTM-only & 9  & 18645  & 52294  & 62415  & 66537 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 9  & 17245  & 49890  & 61232  & 61741 \\
Crafty & 8  & 30682  & 55406  & 67401  & 75834 \\
\hline
 & \mc{4}{c}{genome} \\
HTM-only & 98  & 141077  & 107170  & 296309  & 2345130 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 14027  & 24535  & 46533  & 122295  & 178691 \\
Crafty & 115  & 156604  & 1036466  & 2672553  & 5672160 \\
\hline
 & \mc{4}{c}{intruder} \\
HTM-only & 468  & 1198149  & 3830126  & 10305553  & 23760941 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 651  & 602299  & 2296741  & 4205549  & 6378143 \\
Crafty & 493  & -  & -  & -  & - \\
\hline
 & \mc{4}{c}{kmeans-high} \\
HTM-only & 0  & 233884  & 2693264  & 3048308  & 3359831 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 105  & 313752  & 899223  & 2607749  & 2807000 \\
Crafty & 0  & 174098  & 2935762  & 3493188  & 3825330 \\
\hline
 & \mc{4}{c}{kmeans-low} \\
HTM-only & 0  & 208558  & 807705  & 2693570  & 2765507 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 98  & 378115  & 825831  & 1808057  & 2683844 \\
Crafty & 1  & 88972  & 2711421  & 3078552  & 3421220 \\
\hline
 & \mc{4}{c}{labyrinth} \\
HTM-only & 0  & 272  & 3493  & 2420  & 4127 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 2  & 2  & 271  & 1842  & 3305 \\
Crafty & 0  & 195  & 2223  & 4519  & 8349 \\
\hline
 & \mc{4}{c}{ssca2} \\
HTM-only & 109  & 680  & 2311  & 6708  & 10781 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 67  & 191  & 262224  & 382463  & 412146 \\
Crafty & 799  & 1478  & 3206  & 7060  & 14353 \\
\hline
 & \mc{4}{c}{vacation-high} \\
HTM-only & 236  & 255047  & 897594  & 4342121  & 23353362 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 1572  & 208722  & 1297311  & 2087981  & 4645257 \\
Crafty & 526  & 306659  & 1319070  & 8685459  & 36078629 \\
\hline
 & \mc{4}{c}{vacation-low} \\
HTM-only & 131  & 146852  & 520304  & 2325785  & 8149146 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 429  & 88871  & 748366  & 2011713  & 1850917 \\
Crafty & 234  & 171615  & 924007  & 7052811  & 30557213 \\
\hline
 & \mc{4}{c}{yada} \\
HTM-only & 1126  & 6922591  & 10054364  & 14754128  & 19763010 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 5988  & 5542597  & 8160712  & 10855047  & 15259269 \\
Crafty & 733  & 6482555  & 11516932  & 21056195  & 24196671 \\

    \end{tabular}
    \caption{Number of conflicts on atom.}
    \end{table*}
    

    \begin{table*}
    \small
    \begin{tabular}{@{}l|rrrrr@{}}
    Solution & 1 & 2 & 4 & 8 & 12 \\
    
\hline
 & \mc{4}{c}{bayes} \\
HTM-only & 1245  & 1579  & 2588  & 3055  & 3249 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 1359  & 1392  & 2483  & 3004  & 2997 \\
Crafty & 1945  & 1938  & 2742  & 3249  & 3683 \\
\hline
 & \mc{4}{c}{genome} \\
HTM-only & 3934  & 17611  & 24087  & 30010  & 43880 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 18130  & 15026  & 16056  & 26710  & 26368 \\
Crafty & 10118  & 35101  & 178693  & 388348  & 525640 \\
\hline
 & \mc{4}{c}{intruder} \\
HTM-only & 123998  & 126406  & 144536  & 197889  & 364974 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 134172  & 133650  & 142798  & 159549  & 183731 \\
Crafty & 44192  & -  & -  & -  & - \\
\hline
 & \mc{4}{c}{kmeans-high} \\
HTM-only & 0  & 8596  & 132778  & 147658  & 161654 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 1  & 13631  & 37181  & 128101  & 138133 \\
Crafty & 0  & 5116  & 143388  & 166578  & 183490 \\
\hline
 & \mc{4}{c}{kmeans-low} \\
HTM-only & 0  & 7982  & 33629  & 133660  & 136235 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 1  & 15547  & 34527  & 84642  & 133392 \\
Crafty & 6  & 2812  & 134681  & 148127  & 161641 \\
\hline
 & \mc{4}{c}{labyrinth} \\
HTM-only & 510  & 510  & 510  & 511  & 513 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 509  & 509  & 509  & 510  & 512 \\
Crafty & 510  & 510  & 514  & 602  & 743 \\
\hline
 & \mc{4}{c}{ssca2} \\
HTM-only & 2  & 1  & 1  & 1  & 1 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 7  & 4  & 3  & 2  & 3 \\
Crafty & 1  & 1  & 8  & 10  & 10 \\
\hline
 & \mc{4}{c}{vacation-high} \\
HTM-only & 126966  & 120736  & 125864  & 203135  & 893202 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 167492  & 166950  & 186607  & 164281  & 216277 \\
Crafty & 209804  & 202850  & 267289  & 534505  & 1548202 \\
\hline
 & \mc{4}{c}{vacation-low} \\
HTM-only & 44372  & 43282  & 46397  & 78069  & 261247 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 54370  & 51022  & 56307  & 63852  & 63420 \\
Crafty & 58312  & 109265  & 205185  & 459982  & 1271109 \\
\hline
 & \mc{4}{c}{yada} \\
HTM-only & 392502  & 437794  & 471543  & 621701  & 864800 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 414728  & 423540  & 442536  & 492410  & 664119 \\
Crafty & 420069  & 437466  & 522392  & 979180  & 1184279 \\

    \end{tabular}
    \caption{Number of SGL fallbacks on atom.}
    \end{table*}
    

    \begin{table*}
    \small
    \begin{tabular}{@{}l|rrrrr@{}}
    Solution & 1 & 2 & 4 & 8 & 12 \\
    
\hline
 & \mc{4}{c}{bayes} \\
HTM-only & 0.86975  & 0.90732  & 0.95972  & 0.96617  & 0.96811 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 0.88112  & 0.89805  & 0.95090  & 0.96355  & 0.96502 \\
Crafty & 0.92397  & 0.93569  & 0.96071  & 0.96786  & 0.97375 \\
\hline
 & \mc{4}{c}{genome} \\
HTM-only & 0.11342  & 0.22942  & 0.24943  & 0.29822  & 0.54928 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 0.22266  & 0.21181  & 0.20685  & 0.26841  & 0.26701 \\
Crafty & 0.14033  & 0.29308  & 0.62696  & 0.77991  & 0.84353 \\
\hline
 & \mc{4}{c}{intruder} \\
HTM-only & 0.16234  & 0.17203  & 0.22685  & 0.35355  & 0.52852 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 0.16508  & 0.17108  & 0.19021  & 0.23382  & 0.28638 \\
Crafty & 0.12830  & -  & -  & -  & - \\
\hline
 & \mc{4}{c}{kmeans-high} \\
HTM-only & 0.00053  & 0.47077  & 0.95421  & 0.96388  & 0.97106 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 0.00638  & 0.54903  & 0.80042  & 0.95122  & 0.95783 \\
Crafty & 0.00120  & 0.39184  & 0.95755  & 0.96885  & 0.97663 \\
\hline
 & \mc{4}{c}{kmeans-low} \\
HTM-only & 0.00048  & 0.44577  & 0.77780  & 0.95454  & 0.95664 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 0.01812  & 0.60701  & 0.78499  & 0.91081  & 0.95438 \\
Crafty & 0.00203  & 0.25471  & 0.95255  & 0.95657  & 0.96361 \\
\hline
 & \mc{4}{c}{labyrinth} \\
HTM-only & 0.95238  & 0.95229  & 0.95243  & 0.95335  & 0.95442 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 0.95222  & 0.95204  & 0.95181  & 0.95268  & 0.95410 \\
Crafty & 0.95238  & 0.95221  & 0.95199  & 0.96626  & 0.97942 \\
\hline
 & \mc{4}{c}{ssca2} \\
HTM-only & 0.00083  & 0.00108  & 0.00166  & 0.00350  & 0.00584 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 0.03210  & 0.01832  & 0.01331  & 0.01826  & 0.01962 \\
Crafty & 0.00419  & 0.00341  & 0.00334  & 0.00389  & 0.00456 \\
\hline
 & \mc{4}{c}{vacation-high} \\
HTM-only & 0.69879  & 0.67434  & 0.69289  & 0.77198  & 0.90218 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 0.72017  & 0.70432  & 0.73526  & 0.72482  & 0.77754 \\
Crafty & 0.75180  & 0.72841  & 0.74495  & 0.84532  & 0.93786 \\
\hline
 & \mc{4}{c}{vacation-low} \\
HTM-only & 0.47570  & 0.43599  & 0.47996  & 0.58785  & 0.74213 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 0.47186  & 0.45325  & 0.51321  & 0.56416  & 0.56596 \\
Crafty & 0.50877  & 0.53839  & 0.62634  & 0.79340  & 0.91828 \\
\hline
 & \mc{4}{c}{yada} \\
HTM-only & 0.79948  & 0.81548  & 0.83227  & 0.88210  & 0.91965 \\
DudeTM & -  & -  & -  & -  & - \\
NV-HTM & 0.80655  & 0.80912  & 0.81564  & 0.84317  & 0.89073 \\
Crafty & 0.80815  & 0.81523  & 0.85013  & 0.92607  & 0.94304 \\

    \end{tabular}
    \caption{The percentage of transactions that end in aborts on atom.}
    \end{table*}
    


==> results-macro.tex <==
%auto-ignore
\begin{table}
    \small
    \begin{tabular}{@{}l|rrrr@{}}
    Solution & 1 & 2 & 4 & 6 \\
    
\hline
 & \mc{4}{c}{genome} \\
Regular & 16.99  & 9.80  & 5.24  & 3.61 \\
Write Macro & 16.00  & 10.29  & 5.22  & 3.70 \\
\hline
 & \mc{4}{c}{intruder} \\
Regular & 44.63  & -  & -  & - \\
Write Macro & -  & -  & -  & - \\
\hline
 & \mc{4}{c}{kmeans-high} \\
Regular & 1.26  & 0.67  & 0.34  & 0.29 \\
Write Macro & 0.79  & 0.57  & 0.29  & 0.24 \\
\hline
 & \mc{4}{c}{kmeans-low} \\
Regular & 1.87  & 0.88  & 0.43  & 0.31 \\
Write Macro & 1.21  & 0.72  & 0.38  & 0.27 \\
\hline
 & \mc{4}{c}{ssca2} \\
Regular & 29.06  & 14.70  & 7.50  & 5.25 \\
Write Macro & 28.64  & 14.48  & 7.42  & 5.18 \\
\hline
 & \mc{4}{c}{vacation-high} \\
Regular & 79.42  & 46.22  & 23.68  & 16.88 \\
Write Macro & 69.43  & 38.84  & 19.82  & 14.87 \\
\hline
 & \mc{4}{c}{vacation-low} \\
Regular & 48.64  & 26.40  & 14.47  & 10.77 \\
Write Macro & 37.16  & 19.30  & 11.08  & 8.73 \\
\hline
 & \mc{4}{c}{yada} \\
Regular & 49.60  & -  & -  & - \\
Write Macro & 45.84  & -  & -  & - \\

    \end{tabular}
    \caption{Execution times. Regular is the regular Crafty implementation. Write Macro is Crafty, but with the \code{crafty\_log\_write} function inlined using the macro. Inlining the code makes a significant performance improvement, likely because the code is being compiled with optimizations disabled.}
    \end{table}


==> results-tpcc.tex <==
%auto-ignore

    \begin{table}
    \small
    \begin{tabular}{@{}l|rrrrr@{}}
    Solution & 1 & 2 & 4 & 8 & 12 \\
    
\hline
HTM-only & 173.89k  & 499.33k  & 955.58k  & 1380.79k  & 1567.14k \\
DudeTM & 124.15k  & 271.81k  & 756.29k  & 1192.62k  & 1202.87k \\
NV-HTM & -  & -  & -  & -  & - \\
Crafty & 135.22k  & 302.10k  & 551.55k  & 828.64k  & 872.28k \\

    \end{tabular}
    \caption{1000 transactions per second on TPC-C.}
    \end{table}
    

    \begin{table}
    \small
    \begin{tabular}{@{}l|rrrrr@{}}
    Solution & 1 & 2 & 4 & 8 & 12 \\
    
\hline
HTM-only & 12937  & 757113  & 1476364  & 4835064  & 12438947 \\
DudeTM & 7177  & 840292  & 3991214  & 11067555  & 21888550 \\
NV-HTM & -  & -  & -  & -  & - \\
Crafty & 11265  & 1307121  & 4077486  & 7093203  & 19970512 \\

    \end{tabular}
    \caption{Number of conflicts on TPC-C.}
    \end{table}
    

    \begin{table}
    \small
    \begin{tabular}{@{}l|rrrrr@{}}
    Solution & 1 & 2 & 4 & 8 & 12 \\
    
\hline
HTM-only & 76045  & 28013  & 19643  & 21445  & 118726 \\
DudeTM & 54424  & 42144  & 57277  & 89919  & 268345 \\
NV-HTM & -  & -  & -  & -  & - \\
Crafty & 66591  & 74750  & 142256  & 173508  & 587447 \\

    \end{tabular}
    \caption{Number of SGL fallbacks on TCP-C.}
    \end{table}
    

    \begin{table}
    \small
    \begin{tabular}{@{}l|rrrrr@{}}
    Solution & 1 & 2 & 4 & 8 & 12 \\
    
\hline
 & \mc{4}{c}{tpcc} \\
HTM-only & 58.01\%  & 49.84\%  & 39.83\%  & 43.08\%  & 55.26\% \\
DudeTM & 61.87\%  & 62.26\%  & 48.57\%  & 53.85\%  & 65.85\% \\
NV-HTM & -  & -  & -  & -  & - \\
Crafty & 52.18\%  & 56.33\%  & 51.78\%  & 52.69\%  & 64.40\% \\

    \end{tabular}
    \caption{The percentage of transactions that end in aborts on TPC-C.}
    \end{table}
    

